A Thorough Performance Benchmarking on Lightweight Embedding-based Recommender Systems

Since the creation of the Web, recommender systems (RSs) have been an indispensable mechanism in information filtering. State-of-the-art RSs primarily depend on categorical features, which ecoded by embedding vectors, resulting in excessively large embedding tables. To prevent over-parameterized embedding tables from harming scalability, both academia and industry have seen increasing efforts in compressing RS embeddings. However, despite the prosperity of lightweight embedding-based RSs (LERSs), a wide diversity is seen in evaluation protocols, resulting in obstacles when relating LERS performance to real-world usability. Moreover, despite the common goal of lightweight embeddings, LERSs are evaluated with a single choice between the two main recommendation tasks -- collaborative filtering and content-based recommendation. This lack of discussions on cross-task transferability hinders the development of unified, more scalable solutions. Motivated by these issues, this study investigates various LERSs' performance, efficiency, and cross-task transferability via a thorough benchmarking process. Additionally, we propose an efficient embedding compression method using magnitude pruning, which is an easy-to-deploy yet highly competitive baseline that outperforms various complex LERSs. Our study reveals the distinct performance of LERSs across the two tasks, shedding light on their effectiveness and generalizability. To support edge-based recommendations, we tested all LERSs on a Raspberry Pi 4, where the efficiency bottleneck is exposed. Finally, we conclude this paper with critical summaries of LERS performance, model selection suggestions, and underexplored challenges around LERSs for future research. To encourage future research, we publish source codes and artifacts at \href{this link}{https://github.com/chenxing1999/recsys-benchmark}.

==> 06_future_works.tex <==
% Future works
While our study sheds light on the performance and efficiency of various compression methods, exciting questions remain for future researchers to explore:

\textbf{Suggestions for future LERS research:} First, since most methods currently hinder training efficiency, especially in graph-based collaborative filtering, we suggest that further studies aim to improve this aspect. Second, we recommend incorporating magnitude pruning as a simple yet effective baseline for future research on LERSs. Third, we encourage future researchers to include benchmarks for training and inference efficiency to better demonstrate their methods' effectiveness, particularly for inference, which is often overlooked or unimplemented.

\textbf{Relationship between dataset, compression rate, and method performance:} Our experiments reveal varying performances across recommendation datasets; however, the reasons for these disparities remain unclear. Zhang et al. \cite{zhang2023experimental} observe similar patterns in their CTR task experiments. This opens a critical question for future research on the relationship between dataset characteristics and method performance.

\textbf{Further evaluations:} While our study provides valuable insights, various metrics, such as energy consumption, diversity, and novelty, remain unexplored despite their importance for edge devices \cite{ondevicesurvey2021} and RSs \cite{scells2022reduce}. Common libraries like CodeCarbon \cite{schmidt2021codecarbon} lack support for edge devices. Additionally, our study is limited to Raspberry Pi and Python, which introduces overhead and instability due to garbage collection. Future investigations could expand to other programming languages and edge devices, enabling a more comprehensive benchmark of system efficiency.

==> 07_conclusion.tex <==
In this study, we conducted a comprehensive benchmark for various embedding compression methods on two main tasks of recommendation models. 

\textbf{First}, in the CTR task, all compression techniques have their drawbacks. The performance difference depends on dataset characteristics and sparsity. 
In our evaluation, pruning methods are usually better in the Criteo dataset, while compositional embedding usually has better results in the Avazu dataset. 
Moreover, a method that performs well in one compression rate for a specific dataset is not guaranteed to perform well in another. 
However, in general, the difference between each method is minor. 
So, we recommend starting with QR and PEP for the CTR task as these methods have good training efficiency. Furthermore, in our test, methods within the same category tend to demonstrate similar performance on a given dataset. 
Therefore, after testing simple methods, we can train more complex ones with the category that performed better initially, if necessary.

\textbf{Second}, in the CF task, graph-based models outperform latent-factor-based models; therefore, we suggest focusing on LERSs graph-based models. 
Moreover, the performance drop is more significant in the CF task, which could be due to the more considerable difficulty in compressing CF-based models. 
However, every method still provides competitive results compared to the baseline and methods developed for the CF task. 
Nonetheless, this suggests future work for LERSs should look into their method's performance in CF tasks in general and graph-based models in particular. 

% In our tested methods, PEP generally is the most competitive in various settings
% The simpler methods not under-perform, sometimes worth consideration for simple methods.
\textbf{Third}, PEP typically outperforms other tested methods. Interestingly, simple approaches such as QR and MagPrune perform comparably to more complex ones, especially in lower sparsity rates. 
This indicates that practitioners should use simple methods when dealing with low sparsity rates, as these methods provide a good balance between simplicity and effectiveness.


\textbf{Fourth}, most methods are deployable on edge devices with less memory consumption. Both pruning and compositional approaches create a runtime overhead, which varies based on the deployment environment and specific methods. 
In general, compositional-based methods appears to be a better choice for training efficiency, while pruning is more suitable for edge device settings as the CPU could effectively access unstructured weight matrices. 
Moreover, a reduction in the storage doesn't translate to memory cost in training. 
% Thus, we advocate for further studies to look into training time consumption from methods such as low-precision training.


% We also suggest incorporating magnitude pruning as a general baseline in future research.

% consider  lowering memory cost and reducing training/inference time
% provide idea for eval (energy, ...)


% # Answer to all research questions
% RQ1: Are we able to testify a collection of state-of-the-art LERSs from all three main categories under the same practical evaluation settings?
% No.

% RQ2: What is the transferability between different tasks and sparsity rates?
% - Depend on datasets. At least in two sparsity rate we test.

% RQ3: How is the real-world usability of these LERSs in terms of efficiency and memory consumption during inference?
% For edge devices, and in term of efficiency, pruning based-methods seems to be a better choices, while for workstation settings, uses QR.

% # Shortcoming:
% - Should test more methods from other categories, such as quantization and knowledge distillation
% - Should test more sparsity rates


% # Results need to be confirmed in future
% # The so what (big picture, the implication, speculation)

==> response_figures/avazu_wd.tex <==
\begin{tikzpicture}

\begin{axis}[
    title={\large DCN-Avazu},
    xmin=-0.7, xmax=2.7,
    xtick={0, 1, 2},
    xticklabels={50\%, 80\%, 95\%},
    ybar,
    bar width=12pt,
    width=0.45\textwidth,
    xtick=data,
    ymin=0, 
    % ylabel=Weight Decay,
    xlabel=Sparsity Rate,
]
\addplot table[
    x expr=\coordindex, 
    y=qr
]
{\avazuwd};
\addplot table[
    x expr=\coordindex,
    y=dhe
]
{\avazuwd};


\addplot table[
    x expr=\coordindex,
    y=pep
]
{\avazuwd};


\addplot[
    red, dashed,
    line legend,
    sharp plot
] coordinates {(-1,0.0033289440083949075) (5,0.0033289440083949075)};

\end{axis}
\end{tikzpicture}


==> response_figures/yelp_wd.tex <==
\pgfplotstableread[col sep=comma]{data/yelp_wd.csv}\yelpwd
\pgfplotstableread[col sep=comma]{data/avazu_wd.csv}\avazuwd

\begin{tikzpicture}
% \tikzstyle{every node}=[font=\scriptsize]

\begin{axis}[
    % xticklabel style={
    %     xshift=-10pt,
    % },
    title={\large LightGCN-Yelp},
    xmin=-0.7, xmax=2.7,
    xtick={0, 1, 2},
    xticklabels={50\%, 80\%, 95\%},
    ybar,
    % enlargelimits=0.15,
    bar width=12pt,
    width=0.45\textwidth,
    xtick=data,
    ymin=0, 
    ylabel=Weight Decay,
    xlabel=Sparsity Rate,
    legend style={
        at={(0.8, 1.0)},
        anchor=north,
        legend columns=-1,
        % column sep=0.02\textwidth,
        % row sep=4cm
    },
    % symbolic x coords={50\%, 80\%, 95\%},
    % nodes near coords,
    % nodes near coords align={vertical}
    legend to name=sharedlegend
]
\addplot table[
    x expr=\coordindex, 
    y=qr
]
{\yelpwd};
\addplot table[
    x expr=\coordindex,
    y=dhe
]
{\yelpwd};


\addplot table[
    x expr=\coordindex,
    y=pep
]
{\yelpwd};

\addplot[
    red, dashed,
    line legend,
    sharp plot,
    update limits=false
] coordinates {(-1,0.00975999679147741) (5,0.00975999679147741)};


\legend{QR;, DHE;, PEP;, Original}
\end{axis}
\end{tikzpicture}



==> table-and-figures/figure-criteo-train-v1.tex <==
% Change this to break point figure
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{table-and-figures/criteo-infer-gpu.pdf}
        \caption{Inference. Sparse (*) means we store weight matrix under SparseCSR format.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{table-and-figures/criteo-gpu.pdf}
        \caption[]%
        {Training. Sparse (*) means "gradient with respect to weight matrix will be a sparse tensor"\footnotemark.}
    \end{subfigure}
    \hfill
    \caption{Training and Inference resource usage of Criteo dataset on a workstation.}
    \label{fig:criteo-gpu}
\end{figure*}
\footnotetext{\url{https://pytorch.org/docs/stable/generated/torch.nn.Embedding.html}}


==> table-and-figures/other-backbone-result.tex <==
% \begin{figure}
%     \subcaptionbox{NMF - Yelp2018}
%     {
%         \vspace{-.2cm}
%         \includegraphics[height=0.13\textheight]{table-and-figures/nmf-yelp.pdf}
%     }
%     \subcaptionbox{NMF - Gowalla}
%     {
%         \vspace{-.2cm}
%         \includegraphics[height=0.13\textheight]{table-and-figures/nmf-gowalla.pdf}
%     }
%         \subcaptionbox{DCN - Criteo}
%     {
%         \vspace{-.2cm}
%         \includegraphics[height=0.13\textheight]{table-and-figures/dcn-criteo.pdf}
%     }
%         \subcaptionbox{DCN - Avazu}
%     {
%         \vspace{-.2cm}
%         \includegraphics[height=0.13\textheight]{table-and-figures/dcn-avazu.pdf}
%     }
%     \caption{Other backbones}
%     \label{fig:other-backbones-result}
% \end{figure}


\begin{figure}
    \subcaptionbox{NMF - Yelp2018}
    {
        \vspace{-.2cm}
        \includegraphics[height=0.25\textheight]{table-and-figures/nmf-yelp-bar.pdf}
    }
    \subcaptionbox{NMF - Gowalla}
    {
        \vspace{-.2cm}
        \includegraphics[height=0.25\textheight]{table-and-figures/nmf-gowalla-bar.pdf}
    }
    
    \subcaptionbox{DCN - Criteo}
    {
        \vspace{-.2cm}
        \includegraphics[height=0.25\textheight]{table-and-figures/dcn-criteo-bar.pdf}
    }
        \subcaptionbox{DCN - Avazu}
    {
        \vspace{-.2cm}
        \includegraphics[height=0.25\textheight]{table-and-figures/dcn-avazu-bar.pdf}
    }

    % \subcaptionbox

    \includegraphics[width=0.8\textwidth]{table-and-figures/legend.pdf}
    
    \caption{Other backbones}
    \label{fig:other-backbones-result}
\end{figure}
